Mapping Human Muscle Force to Supernumerary Robotics Device for Overhead Task Assistance

Supernumerary Robotics Device (SRD) is an ideal solution to provide robotic assistance in overhead manual manipulation. Since two arms are occupied for the overhead task, it is desired to have additional arms to assist us in achieving other subtasks such as supporting the far end of a long plate and pushing it upward to fit in the ceiling. In this study, a method that maps human muscle force to SRD for overhead task assistance is proposed. Our methodology is to utilize redundant DoFs such as the idle muscles in the leg to control the supporting force of the SRD. A sEMG device is worn on the operator's shank where muscle signals are measured, parsed, and transmitted to SRD for control. In the control aspect, we adopted stiffness control in the task space based on torque control at the joint level. We are motivated by the fact that humans can achieve daily manipulation merely through simple inherent compliance property in joint driven by muscles. We explore to estimate the force of some particular muscles in humans and control the SRD to imitate the behaviors of muscle and output supporting forces to accomplish the subtasks such as overhead supporting. The sEMG signals detected from human muscles are extracted, filtered, rectified, and parsed to estimate the muscle force. We use this force information as the intent of the operator for proper overhead supporting force. As one of the well-known compliance control methods, stiffness control is easy to achieve using a few of straightforward parameters such as stiffness and equilibrium point. Through tuning the stiffness and equilibrium point, the supporting force of SRD in task space can be easily controlled. The muscle force estimated by sEMG is mapped to the desired force in the task space of the SRD. The desired force is transferred into stiffness or equilibrium point to output the corresponding supporting force.

==> 1-abstract.tex <==
Supernumerary Robotics Device (SRD) is an ideal solution to provide robotic assistance in overhead manual manipulation, especially the tasks including supporting a plate and fitting it in the ceiling in limited space such as compartment. Since two arms are occupied for the overhead task, it is desired to have additional arms to assist us in achieving other subtasks such as supporting the far end of a long plate and pushing it upward to fit in the ceiling. 
In this study, a method that maps human muscle force to SRD for overhead task assistance is proposed. Our methodology is to utilize redundant DoFs such as the idle muscles in the leg to control the supporting force of the SRD. A sEMG device is worn on the operator’s shank where muscle signals are measured, parsed, and transmitted to SRD for control. In the control aspect, we adopted stiffness control in the task space based on torque control at the joint level. We are motivated by the fact that humans can achieve daily manipulation merely through simple inherent compliance property in joint driven by muscles. We explore to estimate the force of some particular muscles in humans and control the SRD to imitate the behaviors of muscle and output supporting forces to accomplish the subtasks such as overhead supporting. The sEMG signals detected from human muscles are extracted, filtered, rectified, and parsed to estimate the muscle force. We use this force information as the intent of the operator for proper overhead supporting force. As one of the well-known compliance control methods, stiffness control is easy to achieve using a few of straightforward parameters such as stiffness and equilibrium point. Through tuning the stiffness and equilibrium point, the supporting force of SRD in task space can be easily controlled. The muscle force estimated by sEMG is mapped to the desired force in the task space of the SRD. The desired force is transferred into stiffness or equilibrium point to output the corresponding supporting force. 
In the preliminary test, we demonstrated the muscle force estimation using sEMG signals from shank, active stiffness control in SRD task space and supporting force control through mapping sEMG to equilibrium point of stiffness in SRD task space. A SRD prototype system is integrated with a sEMG device, a 6-axis force sensor, and a visual odometry camera. Results in the preliminary tests are presented to prove the feasibility of the proposed method.

==> 4-model.tex <==
\section{Model}
\begin{figure}[t]
\centering
\setlength{\abovecaptionskip}{0.1 cm}
\setlength{\belowcaptionskip}{-1 cm}
\includegraphics[width=3.3 in]{figures/general_model.png}
\caption{The general model of SuperArm and operator. In this model, the operator is modeled as part of a manipulator, however, the joint positions and torques of the operator are not controllable.}
\label{fig:general_model}
\end{figure}

The SuperArm configuration is shown in Fig. \ref{fig:SuperArm_concept}, with its base fixed on the back of the operator via a shoulder belt. The total weight of our SuperArm prototype is $5$ kg with joint-level torque control capability. The SuperArm on the operator is inherently modeled as a manipulator with a floating base. A visual odometry device mounted on the base of SuperArm measures the pose of the float base, and a F/T sensor mounted between SuperArm and operator measures the interaction force. 

Our objective is to design a automatic control mechanism in which the SuperArm is able to guarantee human balance, provide sufficient supporting force, and regulate the interaction force between the operator and SuperArm to maintain human body stability. This mechanism considers the operator and SuperArm dynamics and computes desired SuperArm torque inputs based on the operator, SuperArm and environment states. These states are coupled in the dynamic model, and a null space-projection method based on QR decomposition \cite{mistry} is employed to achieve multi-task decoupling. 

A full dynamic model is developed to include the states from operator, SuperArm and the environment. Operator states include interaction forces between the operator and SuperArm, linear and rotational accelerations, linear and rotational velocities. The SuperArm states include joint position, velocity and torque. Environment states include the supporting force from SuperArm. The states and inputs of operator and SuperArm is integrated in this model to take into account the coupled human-SuperArm loop. 

In this section, we will introduce the model in two levels: kinematics and dynamics models. In the kinematics model, the coupling of operator and SuperArm movement is analyzed in two different cases, and their motion relationship is given. In the dynamics model, an analytical solution for SuperArm torques is given to track certain movement of human body and the derivation of related supporting force is also provided.
\vspace{-3mm}
\subsection{Kinematics Model}
The kinematics model studies the coupling of operator and SuperArm motion. Here $q_h \in \Re^{h \times 1}$ and $\tau_h \in \Re^{h \times 1}$ represent human joint position and torque states, respectively; $q_s \in \Re^{s \times 1}$ and $\tau_s \in \Re^{s \times 1}$ represent SuperArm joint position and torque states, respectively; $s$ and $h$ are the number of DoFs of SuperArm and human, respectively. Note that, $\tau_h$ is treated as a state in this model rather than an input. Our objective is to track $q_h$ and regulate $\tau_h$ through control of the SuperArm. Our model only considers the condition $s>h$ since in general manipulator has more DoFs than that of human body to provide the capacity of accomplishing multi-tasks simultaneously. As shown in the frame ${O_{SL}}$ of Fig. \ref{fig:general_model}, $q_h$ depends on $q_s$ and components of $q_h$. Therefore, $q_s$ and $q_h$ obey:

\begin{equation}
    q_h = f(q_{h2}, q_s),
    \label{eq:1}
\end{equation}
where $q_h = [q_{h1}, q_{h2}]^T$ and $q_{h2}$ are coupled states. A closed-kinematic chain exists in the model of Fig. \ref{fig:general_model}, which also imposes an algebraic constraint. In this study, the kinematic model is categorized into two cases: 1) $s = h$ and 2) $s > h$.

Case 1 ($s = h$): in this cases $q_h$ and $q_s$ are decomposed into two components, $q_h = [q_{h1}, q_{h2}]^T$, $q_s = [q_{s1}, q_{s2}]^T$. We design $q_{s2}$ to track $q_{h2}$, i.e. $q_{h2} = K q_{s2}$, where $K$ is selected as a constant coefficient matrix. If $q_{h2}$ includes rotational DoFs, correspondingly $q_{s2}$ is selected from rotation DoFs. Likewise, if $q_{h2}$ includes translation DoFs, correspondingly $q_{s2}$ is selected from translation DoFs. We can select $K$ to cancel $q_{h2}$ in (\ref{eq:1}) so that (\ref{eq:1}) can be simplified to $q_{h1} = f(q_{s1})$. Therefore, the derivative of that equation has,

\begin{equation}
    \dot{q}_{h1} = \hat{J}_{hs} \dot{q}_{s1},
    \label{eq:2}
\end{equation}
where $\hat{J}_{hs}$ is the Jacobian with respect to frame ${O}_{SL}$ as shown in Fig. \ref{fig:general_model}. Combined with $q_{h2} = K q_{s2}$, we have a relationship between $q_h$ and $q_s$ depicted as:
\begin{equation}
    \dot{q}_h = J_{hs} \dot{q}_s =
    \begin{bmatrix}
    \hat{J}_{hs} & O\\
    O & K
    \end{bmatrix} \dot{q}_s,
    \label{eq:3}
\end{equation}
where $J_{hs}$ and $\hat{J}_{hs}$ are square and invertible except at singularity, which is out of scope of this study. This singularity rarely occurs in our implementation. In that case, it makes sense to claim that the singularity does not matter a lot for this letter. From (\ref{eq:3}), $\dot{q}^d_s$ and $q^d_s$ can be computed as:
\begin{equation}
\begin{cases}
\dot{q}^d_s = J^{-1}_{hs} \dot{q}_h,\\
q^d_s - q^a_s = \Delta q_s = J^{-1}_{hs} \dot{q}_h,\\
\end{cases}
\label{eq:4}
\end{equation}
where $q^d_s$ and $q^a_s$ are the desired and actual states respectively.

Case 2 ($s > h$): in the same way as case 1, we still decompose $q_s$ and $q_h$ into $[q_{s1}, q_{s2}]^T$ and $[q_{h1}, q_{h2}]^T$. And $q_{h2}$ is set to be equal to $q_{h2} = K q_{s2}$ with $K$ being a constant coefficient matrix. We have the similar form:
\begin{equation}
    \dot{q}_h = J_{hs} \dot{q}_s = \begin{bmatrix}
    \hat{J}_{hs} & O\\
    O & K
    \end{bmatrix} \dot{q}_s,
    \label{eq:5}
\end{equation}
where $\hat{J}_{hs} \in \Re^{h1 \times s1}$ and $h_1 < s_1$. With svd-based pseudo inverse, we have the inverse of $J_{hs}$ as:

\begin{equation}
    \dot{q}_s = J^{+}_{hs} \dot{q}_h = \begin{bmatrix}
    \hat{J}^{+}_{hs} & O\\
    O & K^{-1}
    \end{bmatrix} \dot{q}_h.
    \label{eq:6}
\end{equation}

Thus $\dot{q}^d_s$ and $q^d_s$ are computed in the same way as case 1:
\begin{equation}
\begin{cases}
\dot{q}^d_s = J^{+}_{hs} \dot{q}_h,\\
q^d_s - q^a_s = \Delta q_s = J^{+}_{hs} \dot{q}_h.\\
\end{cases}
\label{eq:7}
\end{equation}

In this design, SuperArm can spare some DoFs to compensate for the operator's posture. In the simplest way, SuperArm is designed such that all types of DoFs (translational and rotational) correspond to the motion DoFs of operator. However, translational DoFs usually spare large space and most manipulator configuration only includes rotational DoFs. Therefore, it is necessary to discuss the above method. 

In this kinematics model, motion relationship between the operator and SuperArm is discussed with two cases considered. The decoupling method is adopted for SuperArm to track the operator motion.
\vspace{-5mm}
\subsection{Dynamics Model}
A dynamical system is normally formulated as $\dot{x} = f(x, u)$, where $x$ is the system states and $u$ is the input. In this study,  the dynamics with human in the loop is considered and interaction forces between operator and SuperArm as well as the operator's motion states are taken into account. The dynamics is formulated as:

\begin{equation}
    \dot{x} = f(x, u_s, u_h),
    \label{eq:8}
\end{equation}
where $u_s$ and $u_h$ are input of SuperArm and human respectively. $x = [x_s, x_h]^T$ is the system states, including SuperArm sates $x_s$ and human states $x_h$ respectively. Operator is modeled as a part of manipulator and includes 3 rotation DoFs and 3 translation DoFs as shown in Fig. \ref{fig:general_model}. The complete dynamics equation is as:

\begin{equation}
    A \ddot{q} + h = \tau + J^T_c \lambda,
    \label{eq:9}
\end{equation}
where $A$ is inertia matrix, $h$ includes Coriolis force and gravity. $\tau$ is the joint torques of SuperArm and operator. $\lambda$ is the supporting force. $J_c \in \Re^{k \times n}$ is the Jacobian of support point with respect to global frame ${O}$ as shown in Fig. \ref{fig:general_model}. $k$ is the number of DoFs of contact constraint. Since it is assumed that the operator is equivalent to a manipulator with 6 DoFs, of which 3 DoFs are rotational and 3 DoFs are translational, $q$ and $\tau$ are defined as:
\begin{equation}
\begin{cases}
    q = [q_s, q_h]^T, \\
    \tau = [\tau_s, \tau_h]^T,
\end{cases}
\label{eq:10}
\end{equation}
where the subscription $s$ and $h$ represent SuperArm and human respectively. $q_s \in \Re^{s \times 1}$ and $q_h \in \Re^{h \times 1}$. In this study, the condition in which $s \geq h$ is considered. Therefore, QR decomposition of $J^T_c$ has the form as:
\begin{equation}
    J^T_c = Q \begin{bmatrix}
R\\
0
\end{bmatrix},
\label{eq:11}
\end{equation}
where $Q$ is an orthogonal matrix and $Q^T Q = I$, $R \in \Re^{k \times k}$ is an upper triangular matrix with rank of $k$. Therefore, we have:
\begin{equation}
    A \ddot{q} + h = \tau + Q \begin{bmatrix}
R\\
0
\end{bmatrix} \lambda.
\label{eq:12}
\end{equation}

The above equation is decomposed into two parts with $\lambda$ extracted:
\begin{equation}
\begin{cases}
    S_k Q^T ( A \ddot{q} + h - \tau) = R \lambda,\\
    S_{kc} Q^T ( A \ddot{q} + h ) = S_{kc} Q^T \tau,
\end{cases}
\label{eq:13}
\end{equation}
where the selection matrices $S_k$ and $S_{kc}$ are:
\begin{equation}
\begin{cases}
    S_k = [I_k, O_{k \times (n-k)}],\\
    S_{kc} = [O_{(n-k) \times k}, I_{(n-k) \times (n-k)}].
\end{cases}
\label{eq:14}
\end{equation}

Therefore, the contact constrain is canceled from (\ref{eq:14}) and we have:
\begin{equation}
\begin{cases}
    \tau = (S_{kc} Q^T)^{\dag} S_{kc} Q^T ( A \ddot{q} + h ), \\
    \lambda = R^{-1} S_k Q^T N_{kc} ( A \ddot{q} + h),
\end{cases}
\label{eq:15}
\end{equation}
where $(\cdot)^\dag$ is dynamically consistent pseudo-inverse \cite{luis_oussama}, i.e. $W^\dag = A^{-1} W^T (WA^{-1}W^T)^{-1}$. $N_{kc} = I - (S_{kc} Q^T)^{\dag} S_{kc} Q^T$ is the null projection of $S_{kc} Q^T$. $\tau = [\tau_s, \tau_h]^T$, where $\tau_s$ is the joint torque of SuperArm and $\tau_h$ is the joint torque of human. $\ddot{q} = [\ddot{q}_s, \ddot{q}_h]^T$ includes the joint acceleration of SuperArm and human.

The task space above is defined in frame $O_{SL}$ as shown in Fig. \ref{fig:general_model}. The analytical solution given by (\ref{eq:15}) is only one of many feasible ones due to the pseudo inverse used. Therefore, the solution (\ref{eq:15}) is not unique. In this dynamic model, joint torques of SuperArm and human $\tau$ are decoupled with the contact force $\lambda$, which is the supporting force for overhead task. Using (\ref{eq:15}), we can compute the $\tau$ and $\lambda$ using joint acceleration.

This letter aims to regulate the interaction forces and contact forces, which corresponds to $\tau_h$ and $\lambda$. (\ref{eq:15}) is able to provide an efficient solution for joint torque and supporting force. However, this solution does not take human body stability into consideration. To ensure the CoP stability of the operator, a balance control problem is formulated in the next section.

==> 5-control.tex <==
\section{control}
\begin{figure}[ht!]
\centering
\includegraphics[height=2 in]{figures/parietti2016.png}
\caption{Force and moments acting on the SRL system\cite{parietti2016supernumerary}}
\label{fig:parietti2016}
\end{figure}
 In 2015, \cite{parietti2015supernumerary} presented a approach to use SuperLimbs for augmenting human walking stability and reducing the loads on human leg joints. They first investigated the static case, and used SuperLimbs to increase the area of the support polygon of the human-robot system. Then they moved to the dynamic walking case and formulated a gait sequence optimization problem. \cite{parietti2016supernumerary} performed a quasi-static analysis of SuperLimbs for human body support situation as shown in Fig. \ref{fig:parietti2016}. 
When this system is statically balanced, we can have the equilibrium condition as this, 
\begin{equation}
      mge_{z}+F_{h}+J^{T}\tau=0
      \label{eq:parietti2016_1}
\end{equation}
where $F_{h}$ is human generated force and moment, J is the Jacobian matrix. And for stability analysis, it is assumed that $F_h=0$, which means that human does not generate any force other than gravity force of the body. At a equilibrium point $(\Bar{p},\Bar{q})$, (\ref{eq:parietti2016_1}) becomes,
\begin{equation}
      mge_{z}+J^{T}\Bar{\tau}=0
\end{equation}
Combining with joint torque control equation, 
\begin{equation}
      \tau= \Bar{\tau} - K_{q}{\Delta}q
\end{equation}
where, 
\begin{equation}
      {\Delta}q = q - \Bar{q}
\end{equation} and $K_q$ is the real stiffness matrix in joint space,
we can actually have a potential function in the vicinity of the equilibrium point like this,
\begin{equation}
    U = mgz_{c} - \Bar{\tau}^T {\Delta}q + \frac{1}{2}{\Delta}q^{T}K_{q}{\Delta}q
\end{equation}
The quasi-static stability can be examined with the second derivative of this potential function
\begin{equation}
    \frac{d}{dp}(\frac{dU}{dp})^{T} = \frac{d}{dp}(mge_{z}+J^{T}K_{q}{\Delta}q-J^{T}\Bar{\tau})
\end{equation}
To execute the second derivative, two Hessians are needed
\begin{equation}
     E_{z}\overset{\Delta}{=}\frac{de_{z}}{dp}=\left\{\frac{\partial^2z_{c}}{\partial{p_j}\partial{p_k}} \right\}\in \Re^{6\times6}
\end{equation}
\begin{equation}
    H_{i}\overset{\Delta}{=}\left\{\frac{\partial^2q_{i}}{\partial{p_j}\partial{p_k}} \right\} \in \Re^{6\times6},\quad i = 1, \cdots,6.
\end{equation}
And we can evaluate the second derivative the potential function with these Hessians at the equilibrium point where $\tau=\Bar{\tau}$, and the stiffness matrix with which the body is held in equilibrium is given by,
\begin{equation}
\begin{split}
        K_{p}(\Bar{p})&\overset{\Delta}{=}\left.\frac{d}{dp}(\frac{dU}{dp})^{T}\right\vert_{\Bar{p}}\\
        &=\left.(mg\frac{de_z}{dp}+J^{T}K_{q}J-\frac{d}{dp}(J^{T}\tau))\right\rvert_{\Bar{p}}\\
        &=mg\Bar{E_z}+\Bar{J}^{T}K_{q}\Bar{J}-\sum_{i=1}^{6} \Bar{\tau_{i}}\Bar{H_{i}},
\end{split}
\label{eq:parietti2016}
\end{equation}
 To make the SuperLimbs system stable, this stiffness matrix $K_{p}$ in (\ref{eq:parietti2016}) has to be positive semi-definite. Therefore, two control method was provided for stabilizing the human body support system, one is exploit the Hessian term. the third term in (\ref{eq:parietti2016}) and the other is to use joint servo stiffness, which is the second term in (\ref{eq:parietti2016}). 
